Large Language Model-informed ECG Dual Attention Network for Heart Failure Risk Prediction

Heart failure (HF) poses a significant public health challenge, with a rising global mortality rate. Early detection and prevention of HF could significantly reduce its impact. We introduce a novel methodology for predicting HF risk using 12-lead electrocardiograms (ECGs). We present a novel, lightweight dual-attention ECG network designed to capture complex ECG features essential for early HF risk prediction, despite the notable imbalance between low and high-risk groups. This network incorporates a cross-lead attention module and twelve lead-specific temporal attention modules, focusing on cross-lead interactions and each lead's local dynamics. To further alleviate model overfitting, we leverage a large language model (LLM) with a public ECG-Report dataset for pretraining on an ECG-report alignment task. The network is then fine-tuned for HF risk prediction using two specific cohorts from the UK Biobank study, focusing on patients with hypertension (UKB-HYP) and those who have had a myocardial infarction (UKB-MI).The results reveal that LLM-informed pre-training substantially enhances HF risk prediction in these cohorts. The dual-attention design not only improves interpretability but also predictive accuracy, outperforming existing competitive methods with C-index scores of 0.6349 for UKB-HYP and 0.5805 for UKB-MI. This demonstrates our method's potential in advancing HF risk assessment with clinical complex ECG data.

==> algorithms/generic_algorithm.tex <==
\begin{minipage}{\columnwidth}
\begin{algorithm}[H]
    \caption{ Adversarial Example Generation with One-step Power Iteration (K=1).}
    \label{alg: one-step optimization}
\begin{algorithmic}[1]
 \STATE {\bfseries Input:}  Sample mini-batch $\{ \imageinstance\}_{i=1}^{B}$ {from the training dataset: $\dataset_L\; \textrm{or}\; \dataset_U$}, a segmentation network  $\classifier_\theta$
    \STATE {\bfseries Requires:} $\xi$, $\condition$, $\transformation_0$
    \STATE {\bfseries Output:} Adversarial  images $\{\imageinstance_{adv}\}_{i=1}^{B}$
    \FOR {each image $\imageinstance$}
    \STATE Randomly initialize a unit vector $\e_0^{(i)}$ to update the identity transformation $\augment_{\transformation_0}$ with a substantially small transformation: $\augment_{\transformation_0+\xi\e_0^{(i)}}$
    \STATE Take the gradient of the consistency loss $\Distance$ to compute the direction of adversarial transformation $\transformation_{adv}^{(i)}$ and rescale it to ensure it satisfy its constraints $\condition$ using \eqref{Eq: Update transformation}:$\transformation_{adv}^{(i)} \leftarrow \transformation_0+\textit{rescale}(\e_1^{(i)})$
    \STATE Apply the optimized adversarial transformation to get an adversarial augmented image:\\
    $\imageinstance_{adv} =\augment_{\transformation^{(i)}_{adv}}(\imageinstance)$
    \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}


==> figures/lead_attention.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\columnwidth]{figures/images/lead_attention.pdf}
\end{center}
\caption[LeadAttention]{Overview of lead attention module.}
\label{fig:lead_attention}
\end{figure}

==> figures/tmi_example.tex <==
%  When submitting your final paper, your graphics should all be submitted in- dividually in one of these formats (s PostScript (PS), Encapsulated PostScript (.EPS), Tagged Image File Format (.TIFF), Portable Document Format (.PDF), Portable Network Graphics (.PNG), or Metapost (.MPS)) along with the manuscript.

% The online tool, located at http://graphicsqc.ieee.org/, allows authors to upload their graphics in order to check that each file is the correct file format, resolution, size and colorspace; that no fonts are 
 

%%Most charts, graphs, and tables are one column wide (3.5 inches/88 millimeters/21 picas) or page wide (7.16 inches/181 millimeters/43 picas). The maximum depth a graphic can be is 8.5 inches (216 millimeters/54 picas). When choosing the depth of a graphic, please allow space for a caption. Figures can be sized between column and page widths if the author chooses, however it is recommended that figures are not sized less than column width unless when necessary.

%%Labels should appear centered below each subfigure in 8 point Times New Roman font in the format of (a) (b) (c).


\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/images/example.png}
\end{center}
\caption[short-title]{Title.}
\label{fig:example}
\end{figure}
